Temporal-controlled Frame Swap for Generating High-Fidelity Stereo Driving Data for Autonomy Analysis

This paper presents a novel approach, TeFS (Temporal-controlled Frame Swap), to generate synthetic stereo driving data for visual simultaneous localization and mapping (vSLAM) tasks. TeFS is designed to overcome the lack of native stereo vision support in commercial driving simulators, and we demonstrate its effectiveness using Grand Theft Auto V (GTA V), a high-budget open-world video game engine. We introduce GTAV-TeFS, the first large-scale GTA V stereo-driving dataset, containing over 88,000 high-resolution stereo RGB image pairs, along with temporal information, GPS coordinates, camera poses, and full-resolution dense depth maps. GTAV-TeFS offers several advantages over other synthetic stereo datasets and enables the evaluation and enhancement of state-of-the-art stereo vSLAM models under GTA V's environment. We validate the quality of the stereo data collected using TeFS by conducting a comparative analysis with the conventional dual-viewport data using an open-source simulator. We also benchmark various vSLAM models using the challenging-case comparison groups included in GTAV-TeFS, revealing the distinct advantages and limitations inherent to each model. The goal of our work is to bring more high-fidelity stereo data from commercial-grade game simulators into the research domain and push the boundary of vSLAM models.

==> tabs_bkup.tex <==
%****************Table 1*******************
\newcommand{\carlaValidate}{
\begin{table*}[ht]
  \footnotesize
  \centering
  \caption{A comparison of datasets collected from CARLA via TeFS method and the official stereo API, using ORB-SLAM3\cite{ORBSLAM3} stereo odometry evaluation. In all experiments, we only aligned origin with ground truth. All results analyzed using APE, APE\%,and RPE\% provided by evo python package\cite{evo}}
  \label{tbl:carlaValidate}
  \begin{tabular}{l l l|c c c}
    \multirow{2}{*}{\textbf{Map}} & \multirow{2}{*}{\shortstack{\textbf{Trajectory} \\ \textbf{Distance (m)}}} & \multirow{2}{*}{\textbf{Method}} & 
    \multicolumn{3}{c}{\textbf{Evaluate Metrics}} \\
    \cline{4-6}
    &&& APE(m) $\downarrow$ & APE(\%) $\downarrow$ & RPE(m) $\downarrow$ \\ 
    \hline
    \multirow{2}{*}{Town 03} & \multirow{2}{*}{954.41} & Native & \textbf{1.67$\pm$0.59} & \textbf{0.17\%$\pm$0.06\%} & \textbf{0.39$\pm$0.14} \\
    \cline{3-6}
    && TeFS (Ours) & 1.82$\pm$0.65 & 0.19\%$\pm$0.06\% & 0.39$\pm$0.14 \\
    \cline{1-6}
    \multirow{2}{*}{Town 06} & \multirow{2}{*}{957.97} & Native & 4.22$\pm$3.17 & 0.44\%$\pm$0.33\% & 0.31$\pm$0.25 \\
    \cline{3-6}
    && TeFS & \textbf{2.30$\pm$1.67} & \textbf{0.24\%$\pm$0.17\%} & \textbf{0.31$\pm$0.25} \\
    \cline{1-6}
    \multirow{2}{*}{Town 10} & \multirow{2}{*}{950.05} & Native & \textbf{0.98$\pm$0.64} & \textbf{0.10\%$\pm$0.07\%} & \textbf{0.27$\pm$0.22} \\
    \cline{3-6}
    && TeFS & 1.01$\pm$0.63 & 0.10\%$\pm$0.07\% & 0.27$\pm$0.22 \\
    \cline{1-6}
  \end{tabular}
\end{table*}
}

%%%%%%%%%%%%%%%%%Table4%%%%%%%%%%%%%%%%%%%%%
\newcommand{\offroad}{
\begin{table*}[t]
\footnotesize
\caption{Stereo odometry evaluation results of various SOTA vSLAM algorithms on the comparison groups of our GTAV-TeFS dataset. In all experiments, we only aligned origin with ground truth. All results analyzed using APE, APE\%, and RPE\% metrics provided by evo python package\cite{evo}}
\begin{center}
% \resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|lll}
\multirow{2}{*}{\textbf{Weather}} & \multirow{2}{*}{\textbf{Scene}} & \multirow{2}{*}{\textbf{Model}}    & \multicolumn{3}{c}{\textbf{Metrics}} \\
\cline{4-6}
&&& APE(m)   & APE(\%)   & RPE(m)  \\
\hline
 \multirow{9}{*}{Extra Sunny}   & \multirow{3}{*}{City04}   &ORBSLAM3&3.20$\pm$0.85&0.42$\pm$0.11&2.78$\pm$0.16\\% 760.433
&& OV$^2$SLAM&2.53$\pm$1.21&0.33$\pm$0.16&0.06$\pm$0.09\\%759.532
&& VINS Fusion &2.95$\pm$1.36&0.39$\pm$0.18&0.09$\pm$0.26\\%750.691
& \multirow{3}{*}{Offroad01}   &ORBSLAM3&3.16$\pm$1.65&0.26$\pm$0.14&0.11$\pm$0.12\\%1208.307
&& OV$^2$SLAM&4.81$\pm$2.21&0.39$\pm$0.18&0.21$\pm$0.19\\%1206.359
&& VINS Fusion &4.27$\pm$1.73&0.35$\pm$0.14&0.16$\pm$0.25\\%1197.746
& \multirow{3}{*}{Offroad02}   &ORBSLAM3&8.19$\pm$3.95&0.25$\pm$0.12&0.39$\pm$0.26\\%3239.979
&& OV$^2$SLAM&15.47$\pm$12.69&0.48$\pm$0.39&0.36$\pm$2.07\\%3240.932
&& VINS Fusion &15.44$\pm$8.99&0.48$\pm$0.39&0.16$\pm$0.21\\%3232.825
\hline
 \multirow{9}{*}{Cloudy with Rain}   & \multirow{3}{*}{City04}   &ORBSLAM3&2.13$\pm$1.19&0.28$\pm$0.16&0.03$\pm$0.04\\%761.380
&& OV$^2$SLAM&21.01$\pm$9.33&2.77$\pm$1.23&0.29$\pm$2.28\\ %759.441
&& VINS Fusion &3.63$\pm2.00&0.48$\pm$0.26&0.21$\pm$0.48\\%760.843
& \multirow{3}{*}{Offroad01}   &ORBSLAM3&4.19$\pm$2.39&0.35$\pm$0.20&0.07$\pm$0.40\\%1203.250
&& OV$^2$SLAM&6.60$\pm$4.19&0.54$\pm$0.34&0.20$\pm$0.25\\%1216.252m
&& VINS Fusion &49.75$\pm$32.98&4.12$\pm$2.73&0.38$\pm$4.73\\%1207.063
& \multirow{3}{*}{Offroad02}   &ORBSLAM3&9.45$\pm2.77&0.29$\pm$0.09&0.16$\pm$0.14\\%3226.025
&& OV$^2$SLAM&85.62$\pm$65.35&2.65$\pm$2.03&0.14$\pm$0.21\\ %  3225.899
&& VINS Fusion &72.47$\pm$61.96&2.26$\pm$1.93&0.22$\pm$0.70\\%3216.139
\hline
 \multirow{9}{*}{Night Thunder Storm}   & \multirow{3}{*}{City04}   &ORBSLAM3&\multicolumn{3}{c}{Lost track of the map}\\
&& OV$^2$SLAM&54.19$\pm$48.40&7.11$\pm$6.35&0.59$\pm$4.15\\%762.131
&& VINS Fusion &\multicolumn{3}{c}{Map range unreachable}\\
& \multirow{3}{*}{Offroad01}   &ORBSLAM3&\multicolumn{3}{c}{Lost track of the map}\\
&& OV$^2$SLAM&91.90$\pm$45.50&7.57$\pm$3.79&0.29$\pm$2.31\\%1213.447
&& VINS Fusion &\multicolumn{3}{c}{Map range unreachable}\\
& \multirow{3}{*}{Offroad02}   &ORBSLAM3&\multicolumn{3}{c}{Lost track of the map}\\
&& OV$^2$SLAM&160.33$\pm$82.39&4.97$\pm$2.49&0.34$\pm$3.54\\%3228.189m
&& VINS Fusion &\multicolumn{3}{c}{Map range unreachable}\\
\hline

\end{tabular}
\vspace{-.5cm}
\label{tbl:compare}
\end{center}
\end{table*}
}


% %****************Table 2*******************
% \newcommand{\visualSLAM}{
% \begin{table}[h!]
% \footnotesize
%   \centering
%   \caption{A comparison between various SOTA vSLAM enabled by our GTAV-TeFStereo dataset.}
%   \label{tbl:visualSLAM}
%   \begin{tabular}{l|c c c}
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Evaluate Metrics}} \\
%     \cline{2-4}
%     & APE(m) $\downarrow$ & APE(\%) $\downarrow$ & RPE(m) $\downarrow$ \\ 
%     \hline
%     SVO Pro \cite{svo} & 27.05 $\pm$ 13.32 & 0.57\% $\pm$ 0.73\% & 1.06 $\pm$ 0.12 \\
%     OV\begin{math}^{2}\end{math}SLAM \cite{ov2slam} & 170.73 $\pm$ 72.42 & 4.61\% $\pm$ 2.62\% & 4.50 $\pm$ 0.98 \\
%     ORBSLAM3 \cite{ORBSLAM3} & \textbf{5.65 $\pm$ 2.99} & \textbf{0.14\% $\pm$ 0.11\%} & \textbf{0.91 $\pm$ 0.77} \\
%     \hline
%   \end{tabular}
% \end{table}
% }

%****************Table 3*******************
\newcommand{\acvnet}{
\begin{table}[t]
\footnotesize
  \begin{center}
    \caption{A performance comparison of the KITTI Stereo 2015 dataset tested on the learning-based stereo matching algorithm ACVNet \cite{acvnet}. The model was trained multiple times using several synthetic driving datasets including our GTAV-TeFS dataset. For the evaluation metrics, please refer to \cite{acvnet}. All estimation arrays are scale-matched with KITTI ground truth using median.}
    \label{tbl:acvnet}
%    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c c}
        \multirow{2}{*}{\textbf{Dataset}} & 
        \multicolumn{2}{c}{\textbf{Evaluation Metrics}}\\
        \cline{2-3}
        & D1 (\%) $\downarrow$ & Threshold ($\delta>1.0$) $\downarrow$ \\ \hline
        
        \multirow{1}{*}{GTAV-TeFS} & \textbf{28.57\% $\pm$ 16.29\%} & \textbf{65.80\% $\pm$ 12.39\%} \\
        \multirow{1}{*}{CARLA} & 79.79\% $\pm$ 10.20\% & 92.79\% $\pm$ 4.92\% \\
        \multirow{1}{*}{Scene Flow} & 39.37\% $\pm$ 10.86\% & 74.90\% $\pm$ 6.03\% \\ \cline{1-3}
        \hline
        \multirow{1}{*}{Pre-trained} & 14.47\% $\pm$ 8.66\% & 50.20\% $\pm$ 10.24\% \\ \cline{1-3}
    \end{tabular}
    %}
  \end{center}
  \vspace{-.5cm}
\end{table}
}


%%%%%%%%%%%%%%%%%Table4%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\compare}{
% \begin{table*}[t]
% \caption{(Place holder, data needs update)A comparison between various SoAT visual SLAM enabled by our GTAV-TeFStereo dataset.}
% \footnotesize
% \begin{center}
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{lll|lll}
% \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Weather}} & \multirow{2}{*}{\textbf{Model}}    & \multicolumn{3}{c}{\textbf{Metrics}} \\
% \cline{4-6}
%                          &                          &                           & APE(m)   & APE(\%)   & RPE(m)  \\
% \hline
% \multirow{9}{*}{GTAV-TeFStereo}     & \multirow{3}{*}{Sunny}   & ORBSLAM3                 & 28.04$\pm$14.97 &2.88\%$\pm$1.54\%&0.07$\pm$1.13\\
%                          &                          & OV$^2$SLAM&5.47$\pm$1.66    &0.56\%$\pm$0.17\%&0.02$\pm$0.02\\
%                          & & VINS Fusion &6.55$\pm$2.88&0.67\%$\pm$0.30\%&0.12$\pm$0.37\\
%                          & \multirow{3}{*}{Rainy}   & ORBSLAM3&1.71$\pm$1.46 & 0.18\%$\pm$0.15\%&0.03$\pm$0.04\\
%                          &                          & OV$^2$SLAM&4.20$\pm$1.64& 0.43$\pm$0.17&0.02$\pm$0.02\\
%                          && VINS Fusion&4.01$\pm$1.13&0.41$\pm$0.12\%&0.14$\pm$0.31\\
%                          & \multirow{3}{*}{Snowy}   & ORBSLAM3                  &1.86$\pm$1.01&0.19\%$\pm$0.10\%&0.02$\pm$0.02\\
%                          &                          & OV$^2$SLAM                &6.71$\pm$2.75&0.69\%$\pm$0.28\%&0.03$\pm$0.04\\
%                          && VINS Fusion                       &5.97$\pm$2.89&0.62\%$\pm$0.30\%&0.11$\pm$0.28\\ 
% \hline
% \multirow{3}{*}{CARLA}   & \multirow{3}{*}{Sunny}   & ORBSLAM3                   &2.02$\pm$0.32&0.17\%$\pm$0.10\%&0.64$\pm$0.48\\
%                          &                          & OV$^2$SLAM&1.72$\pm$0.41&0.15\%$\pm$0.04\% &0.39$\pm$0.38\\
%                          && VINS Fusion&6.08$\pm$3.11&0.53\%$\pm$0.27\%&1.18$\pm$0.99\\
% \hline
% \multirow{3}{*}{KITTI}   & \multirow{3}{*}{Sunny}   &                               ORBSLAM3&3.20$\pm$1.35&0.15\%$\pm$0.06\%&0.03$\pm$0.15\\
%                          &                          & OV$^2$SLAM&2.33$\pm$1.01&0.11\%$\pm$0.05\%&0.02$\pm$0.13\\
%                          && VINS Fusion&11.04$\pm$4.47&0.50\%$\pm$0.20\%&0.09$\pm$0.07\\
% \hline
% \end{tabular}
% \vspace{-.5cm}
% \label{tbl:compare}
% \end{center}
% \end{table*}
% }



